A Recursive Least Square Method for 3D Pose Graph Optimization Problem

Pose Graph Optimization (PGO) is an important non-convex optimization problem and is the state-of-the-art formulation for SLAM in robotics. It also has applications like camera motion estimation, structure from motion and 3D reconstruction in machine vision. Recent researches have shown the importance of good initialization to bootstrap well-known iterative PGO solvers to converge to good solutions. The state-of-the-art initialization methods, however, works in low noise or eventually moderate noise problems, and they fail in challenging problems with high measurement noise. Consequently, iterative methods may get entangled in local minima in high noise scenarios. In this paper we present an initialization method which uses orientation measurements and then present a convergence analysis of our iterative algorithm. We show how the algorithm converges to global optima in noise-free cases and also obtain a bound for the difference between our result and the optimum solution in scenarios with noisy measurements. We then present our second algorithm that uses both relative orientation and position measurements to obtain a more accurate least squares approximation of the problem that is again solved iteratively. In the convergence proof, a structural coefficient arises that has important influence on the basin of convergence. Interestingly, simulation results show that this coefficient also affects the performance of other solvers and so it can indicate the complexity of the problem. Experimental results show the excellent performance of the proposed initialization algorithm, specially in high noise scenarios.

==> initial.tex <==
To find an initial approximation for the vertices’ orientations, we use similar method adopted by Martinec and Pajdla [?], with the difference that columns of the rotation matrices are not decomposed, and segregated the observations with respect to the reference vertex. Each observation, with respect to the reference vertex, is directly an observation for the orientation of the corresponding vertex. Ideally it means:
\begin{equation}\label{Ras}
    R_i=Z_0^i
\end{equation}
which can be written as
\begin{equation}\label{obsrv0}
    \begin{bmatrix}
        O & \ldots & O & \smash{\overbrace{I}^{i^{th}}} & O & \ldots & O
    \end{bmatrix}
    \mathcal{R} = Z_0^i
\end{equation}
where
\begin{equation}
    \mathcal{R} =
    \begin{bmatrix}
        R_1\\
        \vdots\\
        R_n
    \end{bmatrix}
\end{equation}
$O$ is $3\times 3$ zeros matrix and $I$ is identity $3\times 3$ identity matrix. Other observations between two vertices $i$, $j$ Should satisfy the following equation:
\begin{equation}
    Z_i^j = R_jR_i^T\Longrightarrow Z_i^jR_i-R_j=O
\end{equation}
or equivalently:
\begin{equation}\label{obsrvi}
    \begin{bmatrix}
        O & \ldots & O & \smash{\overbrace{Z_i^j}^{i^{th}}} & O & \smash{\overbrace{-I}^{j^{th}}} & O & \ldots & O
    \end{bmatrix}
    \mathcal{R} = O
\end{equation}

By combining equations \eqref{obsrv0} and \eqref{obsrvi} for all measurements in a matrix, we get
\begin{equation}\label{HRQ}
    \mathcal{H}\mathcal{R}=\mathcal{Q}
\end{equation}

where $\mathcal{H}_{3m\times 3m}$ and $\mathcal{Q}$ are obtained by juxtaposing equations \eqref{obsrv0} and \eqref{obsrvi} for all measurements. By relaxing the constraints of rotation matrices, $R_i\in SO(3)$, the equation \eqref{HRQ} becomes a linear least square problem and can be solved in the closed form
\begin{equation}\label{solvHRQ}
    \mathcal{R} = \left(\mathcal{H}^T\mathcal{H}\right)^{-1}\mathcal{H}^T\mathcal{Q}
\end{equation}

Accordingly the constraints of rotation matrices can be satisfied by solving the following problem
\begin{equation}\label{Rcons}
    R_i^* = \argmin_{R\in SO(3)}\left\|R-R_i\right\|_F
\end{equation}

The closed form solution of \eqref{Rcons} is obtained using singular value decomposition of $R_i$ as follows.
\begin{equation}\label{solvRcons}
    R_i^* = S\,diag([1,1,det(SV^T)])V^T
\end{equation}

where $R_i = S D V^T$ is singular value decomposition of $R_i$.


